Observations of $\Lambda_b^0 \to \Lambda K^+\pi^-$ and $\Lambda_b^0 \to \Lambda K^+K^-$ decays and searches for other $\Lambda_b^0$ and $\Xi_b^0$ decays to $\Lambda h^+h^{\prime -}$ final states

A search is performed for the charmless three-body decays of the $\Lambda_b^0$ and $\Xi_b^0$ baryons to the final states $\Lambda h^+h^{\prime -}$, where $h^{(\prime)} = \pi$ or $K$. The analysis is based on a data sample, corresponding to an integrated luminosity of $3 \rm fb^{-1}$ of $pp$ collisions, collected by the LHCb experiment. The $\Lambda_b^0 \to \Lambda K^+\pi^-$ and $\Lambda_b^0 \to \Lambda K^+K^-$ decays are observed for the first time and their branching fractions and $CP$ asymmetry parameters are measured. Evidence is seen for the $\Lambda_b^0 \to \Lambda \pi^+\pi^-$ decay and limits are set on the branching fractions of $\Xi_b^0$ baryon decays to the $\Lambda h^+h^{\prime -}$ final states.

==> LHCb_HD_comma_separated_author_2016-01-19.tex <==
LHCb collaboration:
R. Aaij, 
C. Abell\'{a}n Beteta, 
B. Adeva, 
M. Adinolfi, 
Z. Ajaltouni, 
S. Akar, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
S. Amerio, 
Y. Amhis, 
L. An, 
L. Anderlini, 
G. Andreassi, 
M. Andreotti, 
J.E. Andrews, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
P. d'Argent, 
A. Artamonov, 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
M. Baalouch, 
S. Bachmann, 
J.J. Back, 
A. Badalov, 
C. Baesso, 
S. Baker, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
V. Batozskaya, 
V. Battista, 
A. Bay, 
L. Beaucourt, 
J. Beddow, 
F. Bedeschi, 
I. Bediaga, 
L.J. Bel, 
V. Bellee, 
N. Belloli, 
I. Belyaev, 
E. Ben-Haim, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
A. Bertolin, 
F. Betti, 
M.-O. Bettler, 
M. van Beuzekom, 
S. Bifani, 
P. Billoir, 
T. Bird, 
A. Birnkraut, 
A. Bizzeti, 
T. Blake, 
F. Blanc, 
J. Blouw, 
S. Blusk, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
A. Borgheresi, 
S. Borghi, 
M. Borisyak, 
M. Borsato, 
M. Boubdir, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
S. Braun, 
M. Britsch, 
T. Britton, 
J. Brodzicka, 
E. Buchanan, 
C. Burr, 
A. Bursche, 
J. Buytaert, 
S. Cadeddu, 
R. Calabrese, 
M. Calvi, 
M. Calvo Gomez, 
P. Campana, 
D. Campora Perez, 
L. Capriotti, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
P. Carniti, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
L. Cassina, 
L. Castillo Garcia, 
M. Cattaneo, 
Ch. Cauet, 
G. Cavallero, 
R. Cenci, 
M. Charles, 
Ph. Charpentier, 
G. Chatzikonstantinidis, 
M. Chefdeville, 
S. Chen, 
S.-F. Cheung, 
M. Chrzaszcz, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
V. Cogoni, 
L. Cojocariu, 
G. Collazuol, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
S. Coquereau, 
G. Corti, 
M. Corvo, 
B. Couturier, 
G.A. Cowan, 
D.C. Craik, 
A. Crocombe, 
M. Cruz Torres, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
E. Dall'Occo, 
J. Dalseno, 
P.N.Y. David, 
A. Davis, 
O. De Aguiar Francisco, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
P. De Simone, 
C.-T. Dean, 
D. Decamp, 
M. Deckenhoff, 
L. Del Buono, 
N. D\'{e}l\'{e}age, 
M. Demmer, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
B. Dey, 
A. Di Canto, 
F. Di Ruscio, 
H. Dijkstra, 
F. Dordei, 
M. Dorigo, 
A. Dosil Su\'{a}rez, 
A. Dovbnya, 
K. Dreimanis, 
L. Dufour, 
G. Dujany, 
K. Dungs, 
P. Durante, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
S. Eisenhardt, 
U. Eitschberger, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
S. Ely, 
S. Esen, 
H.M. Evans, 
T. Evans, 
A. Falabella, 
C. F\"{a}rber, 
N. Farley, 
S. Farry, 
R. Fay, 
D. Fazzini, 
D. Ferguson, 
V. Fernandez Albor, 
F. Ferrari, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
M. Fiore, 
M. Fiorini, 
M. Firlej, 
C. Fitzpatrick, 
T. Fiutowski, 
F. Fleuret, 
K. Fohl, 
M. Fontana, 
F. Fontanelli, 
D. C. Forshaw, 
R. Forty, 
M. Frank, 
C. Frei, 
M. Frosini, 
J. Fu, 
E. Furfaro, 
A. Gallas Torreira, 
D. Galli, 
S. Gallorini, 
S. Gambetta, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garc\'{i}a Pardi\~{n}as, 
J. Garra Tico, 
L. Garrido, 
P.J. Garsed, 
D. Gascon, 
C. Gaspar, 
L. Gavardi, 
G. Gazzoni, 
D. Gerick, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
S. Gian\`{i}, 
V. Gibson, 
O.G. Girard, 
L. Giubega, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
C. Gotti, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
E. Graverini, 
G. Graziani, 
A. Grecu, 
P. Griffith, 
L. Grillo, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
T. Hadavizadeh, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
B. Hamilton, 
X. Han, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
J. He, 
T. Head, 
A. Heister, 
K. Hennessy, 
P. Henrard, 
L. Henry, 
J.A. Hernando Morata, 
E. van Herwijnen, 
M. He\ss, 
A. Hicheur, 
D. Hill, 
M. Hoballah, 
C. Hombach, 
L. Hongming, 
W. Hulsbergen, 
T. Humair, 
M. Hushchyn, 
N. Hussain, 
D. Hutchcroft, 
M. Idzik, 
P. Ilten, 
R. Jacobsson, 
A. Jaeger, 
J. Jalocha, 
E. Jans, 
A. Jawahery, 
M. John, 
D. Johnson, 
C.R. Jones, 
C. Joram, 
B. Jost, 
N. Jurik, 
S. Kandybei, 
W. Kanso, 
M. Karacson, 
T.M. Karbach, 
S. Karodia, 
M. Kecke, 
M. Kelsey, 
I.R. Kenyon, 
M. Kenzie, 
T. Ketel, 
E. Khairullin, 
B. Khanji, 
C. Khurewathanakul, 
T. Kirn, 
S. Klaver, 
K. Klimaszewski, 
M. Kolpin, 
I. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Kozeiha, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
P. Krokovny, 
F. Kruse, 
W. Krzemien, 
W. Kucewicz, 
M. Kucharczyk, 
V. Kudryavtsev, 
A. K. Kuonen, 
K. Kurek, 
T. Kvaratskheliya, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
G. Lanfranchi, 
C. Langenbruch, 
B. Langhans, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
E. Lemos Cid, 
O. Leroy, 
T. Lesiak, 
B. Leverington, 
Y. Li, 
T. Likhomanenko, 
R. Lindner, 
C. Linn, 
F. Lionetto, 
B. Liu, 
X. Liu, 
D. Loh, 
I. Longstaff, 
J.H. Lopes, 
D. Lucchesi, 
M. Lucio Martinez, 
H. Luo, 
A. Lupato, 
E. Luppi, 
O. Lupton, 
N. Lusardi, 
A. Lusiani, 
X. Lyu, 
F. Machefert, 
F. Maciuc, 
O. Maev, 
K. Maguire, 
S. Malde, 
A. Malinin, 
G. Manca, 
G. Mancinelli, 
P. Manning, 
A. Mapelli, 
J. Maratas, 
J.F. Marchand, 
U. Marconi, 
C. Marin Benito, 
P. Marino, 
J. Marks, 
G. Martellotti, 
M. Martin, 
M. Martinelli, 
D. Martinez Santos, 
F. Martinez Vidal, 
D. Martins Tostes, 
L.M. Massacrier, 
A. Massafferri, 
R. Matev, 
A. Mathad, 
Z. Mathe, 
C. Matteuzzi, 
A. Mauri, 
B. Maurin, 
A. Mazurov, 
M. McCann, 
J. McCarthy, 
A. McNab, 
R. McNulty, 
B. Meadows, 
F. Meier, 
M. Meissner, 
D. Melnychuk, 
M. Merk, 
A Merli, 
E Michielin, 
D.A. Milanes, 
M.-N. Minard, 
D.S. Mitzel, 
J. Molina Rodriguez, 
I.A. Monroy, 
S. Monteil, 
M. Morandin, 
P. Morawski, 
A. Mord\`{a}, 
M.J. Morello, 
J. Moron, 
A.B. Morris, 
R. Mountain, 
F. Muheim, 
D. M\"{u}ller, 
J. M\"{u}ller, 
K. M\"{u}ller, 
V. M\"{u}ller, 
M. Mussini, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
A. Nandi, 
I. Nasteva, 
M. Needham, 
N. Neri, 
S. Neubert, 
N. Neufeld, 
M. Neuner, 
A.D. Nguyen, 
C. Nguyen-Mau, 
V. Niess, 
S. Nieswand, 
R. Niet, 
N. Nikitin, 
T. Nikodem, 
A. Novoselov, 
D.P. O'Hanlon, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
C.J.G. Onderwater, 
B. Osorio Rodrigues, 
J.M. Otalora Goicochea, 
A. Otto, 
P. Owen, 
A. Oyanguren, 
A. Palano, 
F. Palombo, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
L.L. Pappalardo, 
C. Pappenheimer, 
W. Parker, 
C. Parkes, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
C. Patrignani, 
A. Pearce, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
P. Perret, 
L. Pescatore, 
K. Petridis, 
A. Petrolini, 
M. Petruzzo, 
E. Picatoste Olloqui, 
B. Pietrzyk, 
M. Pikies, 
D. Pinci, 
A. Pistone, 
A. Piucci, 
S. Playfer, 
M. Plo Casasus, 
T. Poikela, 
F. Polci, 
A. Poluektov, 
I. Polyakov, 
E. Polycarpo, 
A. Popov, 
D. Popov, 
B. Popovici, 
C. Potterat, 
E. Price, 
J.D. Price, 
J. Prisciandaro, 
A. Pritchard, 
C. Prouve, 
V. Pugatch, 
A. Puig Navarro, 
G. Punzi, 
W. Qian, 
R. Quagliani, 
B. Rachwal, 
J.H. Rademacker, 
M. Rama, 
M. Ramos Pernas, 
M.S. Rangel, 
I. Raniuk, 
G. Raven, 
F. Redi, 
S. Reichert, 
A.C. dos Reis, 
V. Renaudin, 
S. Ricciardi, 
S. Richards, 
M. Rihl, 
K. Rinnert, 
V. Rives Molina, 
P. Robbe, 
A.B. Rodrigues, 
E. Rodrigues, 
J.A. Rodriguez Lopez, 
P. Rodriguez Perez, 
A. Rogozhnikov, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
J. W. Ronayne, 
M. Rotondo, 
T. Ruf, 
P. Ruiz Valls, 
J.J. Saborido Silva, 
N. Sagidova, 
B. Saitta, 
V. Salustino Guimaraes, 
C. Sanchez Mayordomo, 
B. Sanmartin Sedes, 
R. Santacesaria, 
C. Santamarina Rios, 
M. Santimaria, 
E. Santovetti, 
A. Sarti, 
C. Satriano, 
A. Satta, 
D.M. Saunders, 
D. Savrina, 
S. Schael, 
M. Schiller, 
H. Schindler, 
M. Schlupp, 
M. Schmelling, 
T. Schmelzer, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M. Schubiger, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
A. Semennikov, 
A. Sergi, 
N. Serra, 
J. Serrano, 
L. Sestini, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
V. Shevchenko, 
A. Shires, 
B.G. Siddi, 
R. Silva Coutinho, 
L. Silva de Oliveira, 
G. Simi, 
M. Sirendi, 
N. Skidmore, 
T. Skwarnicki, 
E. Smith, 
I.T. Smith, 
J. Smith, 
M. Smith, 
H. Snoek, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
P. Spradlin, 
S. Sridharan, 
F. Stagni, 
M. Stahl, 
S. Stahl, 
S. Stefkova, 
O. Steinkamp, 
O. Stenyakin, 
S. Stevenson, 
S. Stoica, 
S. Stone, 
B. Storaci, 
S. Stracka, 
M. Straticiuc, 
U. Straumann, 
L. Sun, 
W. Sutcliffe, 
K. Swientek, 
S. Swientek, 
V. Syropoulos, 
M. Szczekowski, 
T. Szumlak, 
S. T'Jampens, 
A. Tayduganov, 
T. Tekampe, 
G. Tellarini, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
S. Tolk, 
L. Tomassetti, 
D. Tonelli, 
S. Topp-Joergensen, 
E. Tournefier, 
S. Tourneur, 
K. Trabelsi, 
M. Traill, 
M.T. Tran, 
M. Tresch, 
A. Trisovic, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
A. Ukleja, 
A. Ustyuzhanin, 
U. Uwer, 
C. Vacca, 
V. Vagnoni, 
S. Valat, 
G. Valenti, 
A. Vallier, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
C. V\'{a}zquez Sierra, 
S. Vecchi, 
M. van Veghel, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
M. Vieites Diaz, 
X. Vilasis-Cardona, 
V. Volkov, 
A. Vollhardt, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
J.A. de Vries, 
R. Waldi, 
C. Wallace, 
R. Wallace, 
J. Walsh, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
D. Websdale, 
A. Weiden, 
M. Whitehead, 
J. Wicht, 
G. Wilkinson, 
M. Wilkinson, 
M. Williams, 
M.P. Williams, 
M. Williams, 
T. Williams, 
F.F. Wilson, 
J. Wimberley, 
J. Wishahi, 
W. Wislicki, 
M. Witek, 
G. Wormser, 
S.A. Wotton, 
K. Wraight, 
S. Wright, 
K. Wyllie, 
Y. Xie, 
Z. Xu, 
Z. Yang, 
H. Yin, 
J. Yu, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
L. Zhang, 
Y. Zhang, 
A. Zhelezov, 
Y. Zheng, 
A. Zhokhov, 
L. Zhong, 
V. Zhukov, 
S. Zucchelli

